Evaluating tamper resistance of digital forensic artifacts during event reconstruction

Event reconstruction is a fundamental part of the digital forensic process, helping to answer key questions like who, what, when, and how. A common way of accomplishing that is to use tools to create timelines, which are then analyzed. However, various challenges exist, such as large volumes of data or contamination. While prior research has focused on simplifying timelines, less attention has been given to tampering, i.e., the deliberate manipulation of evidence, which can lead to errors in interpretation. This article addresses the issue by proposing a framework to assess the tamper resistance of data sources used in event reconstruction. We discuss factors affecting data resilience, introduce a scoring system for evaluation, and illustrate its application with case studies. This work aims to improve the reliability of forensic event reconstruction by considering tamper resistance.

==> text-blocks.tex <==
Similarly to traditional forensic science crime scenes, digital forensic `crime scenes' are influenced by the passing of time. As examiners typically inspect data after a certain interval of time has elapsed, data is affected by intrinsic events that are due to the normal course of happenings \cite{jaquet-chiffelle_formalized_2021}. For example, a timestamp relied on may have been updated by another process. Although this problem cannot be directly addressed, i.e., stored data on a system will necessarily be influenced by the environment and the passing of time, it does need to be taken into consideration during event reconstruction. 

The interpretation of the information contained in timelines remains a challenge rarely addressed. One possible reason for this may be that the causes affecting interpretation during event reconstruction and the resulting evaluation are not fully understood. Given that the events we are trying to reconstruct happened in the past and cannot be revisited, relevant data is intermingled with an ensemble of other data generated by other activities or in some cases by the process of investigation itself \cite{roux_sydney_2022}. Consequently, interpreting the information requires careful consideration of the reliability of the data at hand. Especially, when relevant data has been tampered with, the risk of misinterpretation is increasing \cite{CASEY2020200888}. 

Potential tampering of data is an important consideration as it may lead to substantial misinterpretations. It is typically utilized by active opponents to hide activities by various means, e.g., backdating, erasing, encrypting, or even wiping \cite{CASEY2020200888}. Manipulations may affect file system timestamps used to infer events, or the content of files themselves \sout{(e.g., the content of a PDF file)}. 
While specific inconsistencies such as event logs entries or the presence of certain anti-forensic software may indicate possible manipulations, tampering may not always be easy to detect \cite{palmbach_artifacts_2020}. Additionally, existing anti-forensic tools may also recreate normal user activities in order to hide/obfuscate their activity \cite{galhuber_time_2021}.  Hence, detecting irregularities is crucial for investigators as highlighted recently in the World Anti-Doping Agency v.~Russian Anti-Doping Agency case \cite{wada2020cas}. 

